UDA-COPE: Unsupervised Domain Adaptation for Category-level Object Pose Estimation

Learning to estimate object pose often requires ground-truth (GT) labels, such as CAD model and absolute-scale object pose, which is expensive and laborious to obtain in the real world. To tackle this problem, we propose an unsupervised domain adaptation (UDA) for category-level object pose estimation, called UDA-COPE. Inspired by recent multi-modal UDA techniques, the proposed method exploits a teacher-student self-supervised learning scheme to train a pose estimation network without using target domain pose labels. We also introduce a bidirectional filtering method between the predicted normalized object coordinate space (NOCS) map and observed point cloud, to not only make our teacher network more robust to the target domain but also to provide more reliable pseudo labels for the student network training. Extensive experimental results demonstrate the effectiveness of our proposed method both quantitatively and qualitatively. Notably, without leveraging target-domain GT labels, our proposed method achieved comparable or sometimes superior performance to existing methods that depend on the GT labels.

==> figure/fig_teaser/fig_teaser.tex <==
%Figure
\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figure/fig_teaser/teaser.pdf}
% \vspace{1.0mm}
\caption{\textbf{Learning scheme of our unsupervised domain adaptation for category-level object pose estimation (UDA-COPE).} Our method is trained using pseudo label from teacher model. Our proposed pose aware confidence filtering (PACF) improves the pseudo label.}
\label{fig:teaser}
\end{center}
\end{figure}

==> section/9-backup.tex <==
We give consistency loss for 2D logit and 3D logit with dual head structures. We set the loss weights $0.1$ for xMUDA loss compared to cross entropy loss for the student network. \Tref{tab:ablation_study_all} shows that xMUDA helps to improve the $5^{\circ}, 5$cm metric for all branches. It can be seen that the method of xMUDA gives slight performance improvement in category-level object pose estimation task.
After applying pose-aware bidirectional filtering for pseudo labels (FPL) on BL3, our RGB-D method slightly improve at $5^{\circ}, 2$cm metric than xMUDA. Like xMUDA, 3D IOU 50 shows a slight performance drop on RGB-D based method, which indicates FPL and xMUDA still show a performance drop due to the domain gap. After our proposed self-supervised loss (SSL)~\eqref{self_supervised_learning}, our method significantly improves from the baseline. And it indicates that our proposed loss reduces the domain gap between source and target using pose aware geometry. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent{\textbf{Synthetic and Real dataset.}} We evaluate our method when the synthetic and real data access are available for training. We compare our method with the supervised methods and unsupervised method. The results are summarized on \Tref{tab:real_sota_rgb_comparision}. Our RGB based method outperforms the RGB based supervised methods~\cite{wang2019normalized, Tian2020prior}, even our method doesn't use the real labeled data. Our approach also outperforms CPS++~\cite{manhardt2020cps++} by a large margin 9.2\% for the 3D IOU (75).  Compared to training synthetic only results on \Tref{tab:source_only_comparison}, CPS++~\cite{manhardt2020cps++} decrease 0.6\% at $5^{\circ}, 5$cm metric from 25.8\% to 25.2\% after using unlabeled real dataset. In contrast, our RGB model improves 8.7\% from 18.3\% to 27\%. This improvement is better than a supervised method, NOCS (+6.4\%). 
% Note that CPS++ use additional their own dataset(30k) with NOCS REAL trainingset (4.3k).

% \Tref{tab:real_sota_rgbd_comparison} shows the comparison with the RGB-D based state-of-the-art methods. 
% Our method achieved the best performance on the 3D IOU (50) metric. Compared to other strong supervised based methods, our approach shows some par results and sometimes outperforms them without any real labeled. Specifically, compared to synthetic only, Our model(RGB-D) significantly improves the mAP by 7.4\% for $5^{\circ}, 2$cm metric using unlabeled real dataset. The improvement is close to supervised Shape Prior(RGB-D) that increases by 8.1\%. It shows that our proposed UDA-COPE are valid when the real dataset doesn't have labels.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
lower performance in $5^{\circ}, 2$cm in strict metric. However, the 3D IOU 75 is close to the method, even better than it. This indicates that our pseudo label has given less accurate pose annotations compared to human based labels. However, except for the SGPA~\cite{chen2021sgpa}, our RGB-D method achieves the best performance in $5^{\circ}, 2$ metric, our method shows comparable results comparing the supervised methods. We believe that there is room for our improvement when additionally using shape prior information like them~\cite{Tian2020prior, wang2021category, chen2021sgpa}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method use the filtered align depth points as a ground truth for training teacher network. \Tref{tab:ablation_study_all} shows 1.2\% improvements at $10^{\circ}, 2$cm metric. The result indicates that momentum update is no enough for teacher training. When we jointly update teacher network using momentum update and self-supervised learning loss, it improves 3.9\% at $5^{\circ}, 2$cm metric on RGB-D branch. It shows that jointly training the teacher network to give better pseudo labels for the student network. Our proposed methods outperform the xMUDA~\cite{jaritz2020xmuda} in the category-level object pose estimation task.

 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Most of the previous methods~\cite{jaritz2020xmuda, li2019bidirectional} give training signals to the single modality (RGB) for pseudo label. For example, xMUDA~\cite{jaritz2020xmuda} gives training signals only fused (RGB-D) branch for training loss, despite using a 2D branch and 3D branch. Compared to previous works, our method gives training signals to all signals and each branch becomes more guided to ground-truth and it makes RGB-D branch also increase the performance. We denote giving all modality signals as AM in the ~\Tref{tab:ablation_study_all}. It shows that all modality loss with pseudo labels (PL+AM) significantly increase the overall performance. 
We also compare the momentum update~\cite{he2019moco} to make teacher estimate more high quality pseudo labels. It shows that marginally improves in Depth and RGB-D branches. In RGB branch marginally decrease the performance 0.7\% at 3D IOU (75).

% \noindent{\textbf{All Modality Loss.}}
% One naive strategy to train our network is computing the loss only for the RGB-D estimation same as Xmuda~\cite{jaritz2020xmuda}. However, our network is consists of three estimations from each modality (RGB, Depth, RGB-D) and it makes computing losses for each ouputs. We denote it, as all modality loss. \Tref{tab:ablation_study_all} shows that this simple loss strategy gives better performance than single loss. We achieves significant improvements at  $5^{\circ}, 2$cm metric (24.8\% compared to 13.5\%).

 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 In contrast to existing supervised RGB-D methods, our method achieved the best performance on the 3D IOU (50) metric, even not using 6D object pose labels and NOCS map labels. Note that Shape Prior~\cite{Tian2020prior}, CR-Net~\cite{wang2021category}, SGPA~\cite{chen2021sgpa} use the additional category-wise shape prior information to improve the pose estimation during inference. Despite the lack of additional shape prior in our method, our RGB-D based method outperforms the Shape Prior~\cite{Tian2020prior}, and CR-Net~\cite{wang2021category}. Comparing only the 
method of RGB based supervised methods~\cite{wang2019normalized, Tian2020prior}, our RGB based method achieves the state-of-the arts.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \noindent{\textbf{Synthetic dataset Only}}  We compare our network with other state-of-the-art methods that train from only synthetic dataset and evaluate the results on the REAL275 dataset. \Tref{tab:source_only_comparison} summarizes the results. Our RGB based method achieve state-of-the-arts at 3D IOU(50) metrics, even outperforms the RGB-D based method~\cite{Tian2020prior} by a margin of 8.9\%. Compared to CPS++~\cite{manhardt2020cps++}, our RGB based show lower performance at $5^{\circ}, 5$cm. Our RGB-D based method better performance than our single modality based method. The performance of $10^{\circ}, 2$cm significantly increased from 37.6\% (RGB) to 57.1\% (RGB-D). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%($\mathcal{A}_{2D}$, $\mathcal{A}_{3D}$) 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We use the same network structure for teacher and student models, but do not share the networks' weights. Our network has 2D, 3D branches that do not share features and add a fusion branch that shares the 2D features $F_{2D}$ and 3D features $F_{3D}$. We use the MinUNet34~\cite{choy20194d} for 3D branch and PSPNet~\cite{zhao2017pyramid} with ResNet34~\cite{he2016deep} for 2D branch. For the fused branch, we simply fuse(concat) each modality feature ($F_{2D}$ ,$F_{3D}$) and estimate the NOCS map $\mathcal{N}$ from fused feature $F_{RGB-D}$. Each features ($F_{2D}$ ,$F_{3D}$, $F_{RGB-D}$) regress NOCS map $\mathcal{N}$ after four MLP layers. We denote each NOCS map regression as $\mathcal{N}_{2D}$, $\mathcal{N}_{3D}$, $\mathcal{N}_{RGB-D}$, which depend on feature property.
% NOCS representation을 표현하는 방식 
% [Regression + Classification] 중에서 선택한 이유 설명 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fused의 목적과 구조
Previous methods~\cite{Tian2020prior, chen2020cass, chen2021sgpa, lin2021dualposenet} use the PointNet~\cite{qi2017pointnet,qi2017pointnet++} structure as the baseline of the 3D branch. However, we observed that the PointNet structure has lacked local point information and it dramatically decreased the performance without any RGB guidance on category-level object pose task. To mitigate the significant performance drop on a 3D branch, we first adopt the Mink34-U-Net ~\cite{choy20194d} as the baseline for the category-level pose estimation task. We initialize our Mink34-U-Net using pretrained weights trained from ScanNet~\cite{dai2017scannet} except the last layer. Because the last layer the output channel ($C$) is different from the original network.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We choose the $C$ channel bin based representation for two reasons. As reported by Wang~\etal~\cite{wang2019normalized}, the 32 bins get the best performance than any others and it can also potentially regard as the confidence of NOCS, such as segmentation~\cite{jaritz2020xmuda}. In our method, one naive approach is calculating the pseudo label confidence using softmax probability. We analyze this confidence in \Sref{subsec:ablation_study}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The self-supervised loss (PACF-S) can adapt after filtered the outliers using PACF. After filtering the outliers or noisy pseudo NOCS, we minimize the distance of transformed depth point cloud and predicted pseudo NOCS labels. We converts the transformed depth point cloud as 32 bins NOCS representation for training. \Sref{subsec:ablation_study} shows that PACF-S helps to improve the student network. To more integrate with teacher and student network each other, our method also uses the recent momentum update~\cite{chen2018road, zheng2021rectifying, zheng2019unsupervised} to update student knowledge to the teacher model (\Sref{tab:ablation_study_rgb}).
% todo add: equation


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% 전체적인 방법론 설명
% 1.Detection/Segmentation Given이고 Pose and size에 대한 부분만 풀겠다
% Network 설명 + Pose Aware한 모듈 설명

% \JS{I think part of the sentences below should move the last paragraph in related works.}
% \TY{Most of the recent category-level object pose and size methods~\cite{wang2019normalized, Tian2020prior, wang2021category, chen2021sgpa} use the dense normalized object coordinate space (NOCS) representation as a basic concept to estimate pose and size. Follow by the previous works, we use the NOCS representation and this is also domain invariant representation. Our work concentrates on how to make high quality pseudo NOCS labels using the RGB-D. Note that our method only considers the NOCS pseudo labels, does not cover the pseudo segmentation labels instead uses the pre-trained off-the-shelf 2D detectors(\eg, Mask R-CNN~\cite{he2017mask}) to crop the RGB image and sample the point clouds.}
%
% \JS{Note that our method only considers the NOCS pseudo labels, does not cover the pseudo segmentation labels instead uses the pre-trained off-the-shelf 2D detectors (\eg, Mask R-CNN~\cite{he2017mask}) to crop the RGB image and sample the point clouds same as previous works~\cite{Tian2020prior, chen2020cass, wang2021category, chen2021sgpa, lin2021dualposenet}.}
%
% we first introduce our unsupervised domain adaptation for category-level object pose estimation (UDA-COPE) architecture in \Sref{subsec:network_architecture} and explains the learning schemes in \Sref{subsec:learning_scheme}. And then, we introduce our proposed pose aware confidence-based filtering (PACF) and self-supervised loss (PACF-S) for high quality pseudo labels in \Sref{fig:pose_aware_pseudo_labels}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{equation}
\label{eq:consistency}
 L_{CE}(\mathcal{M}_t (\mathcal{A}_{3D_a}(\mathcal{P}_c), \\
 \mathcal{A}_{2D_a}(\mathcal{I}_c)), \mathcal{M}_t (\mathcal{A}_{3D_b}(\mathcal{P}_c), \mathcal{A}_{2D_b}(\mathcal{I}_c)))
\end{equation}

We first introduce the most recent studies in category-level object pose estimation. Afterwards, we discuss important methods using unlabeled real data. Lastly, we take a brief look at domain adaptation in the field of 6D pose and multi-modal unsupervised domain adaptation methods.


% [Real data를 만들기 어려운 것을 해결하기 위한 관련된 방법들 설명]
%   1. Instance level에서의 방법들  
%   2. Category-level에서의 방법들
        % 기존의 방법: Complete 3D Shape + Rendering 방법에 의존 
        % 문제점: Complete 3D Shape을 observation만 가지고 reconstruction하는게 어렵다 
% 우리의 방법른: 3D shape dependency없이 RGB-D만을 사용해서 이 문제를 해결한다.

% To overcome this problem in the instance-level object pose methods, many works\cite{peng2019pvnet, zakharov2019dpod, kehl2017ssd, park2019pix2pose, wang2020self6d} have tried to render images to get various free 6D pose data using the given 3D CAD models. However, there is significant domain gap (appearance, illumination conditions) between 3D models and real objects and these methods can not deal unseen objects.
% Only a few works~\cite{manhardt2020cps++, zakharov2020autolabeling} have been addressed in category-level object pose. Similar to instance-level, they render image/mask/depth based on the reconstructed 3D shape (mesh~\cite{manhardt2020cps++} or sign distance fields~\cite{zakharov2020autolabeling}) using additional networks \cite{groueix2018papier, park2019deepsdf}. However, estimating unseen 3D shapes from partial observation is a challenge task, and hard to extend multi-class shape estimation with a single network. 
% Therefore, the performance is greatly affected by how accurately and the 3D shape is accurately reconstructed. Moreover, their methods use depth information for a loss function but, they don't fully utilize the RGB-D data and mostly rely on a single RGB for network input. To remedy these problems, the most straightforward solution would be to get rid of the dependency on the complete 3D shape and  utilize RGB-D sensor with domain invariant NOCS representation. 
% \JS{To address the issue, we introduce ... previous studies~\cite{} adopt data augmentation through image rendering from the given 3D CAD models. However, there is a significant domain gap between real-world images and rendered images with respect to the illumination conditions and appearance. Moreover, instance-level methods cannot generalize toward unmet objects.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Recent deep learning-based category-level object pose and size estimation studies rely on real-world labeled data for supervised training. However, it is very laborious and expensive to obtain adequate 6D pose and size annotations. To tackle this problem, we propose unsupervised domain adaptation (UDA) for category-level object pose estimation (UDA-COPE) to train deep networks without any pose and size real labels using RGB-D data. %\JS{without real-world ground truth using RGB-D data.}
Inspired by recent multi-modal UDA techniques, we concentrate on the way of obtaining domain-invariant pseudo labels in normalized object coordinate spaces (NOCS). To this end, we introduce pose-aware confidence-based filtering to filter inaccurate pseudo labels and improve the pseudo label using self-supervision loss with momentum update. Extensive experiments demonstrate that our method robustly infers the poses and sizes of unseen object instances in real environments without using any 6D pose and size of real labels.
Extensive experiments demonstrate our method robustly infers unmet objects' poses and sizes. Moreover, our method reaches par with fully supervised methods with no use of real-world labels.


% For instance object pose estimation, Self6D~\cite{wang2020self6d} only use extra modality (depth) for the training time. CPS++~\cite{manhardt2020cps++} extends Self6D to category-level object pose estimation. It still mainly used additional modality for the training. Otherwise, we use full modalities as network input for category-level object pose estimation.



% \JS{@TY, Why mention? too much for related works. $\rightarrow$}
% \TY{To overcome this problem, directly training a model using only the source domain (synthetic data) would be an alternatives. However it often leads to over-fitting, causing reduce performance when recognizing in the target domain (real data). Braiding the domain gap between synthetic and real data is a crucial task in 6D pose estimation.}
% \JS{@TY, ???? sudden instance-level ???? $\rightarrow$}
% To tackle this problem in the instance-level object pose estimation, many works\cite{peng2019pvnet, zakharov2019dpod, kehl2017ssd, park2019pix2pose, wang2020self6d} have been tried to render images to get various free 6d pose data using given the 3D CAD model. 




\begin{comment}
% Inspired by xMUDA~\cite{jaritz2020xmuda}, we use a 3-stream architecture to address the domain gap and self-training strategy with pseudo-labels. Compared to xMUDA, our UDA-COPE uses NOCS representation and focus on how to make high quality pseudo label for category-level pose estimation task. To handle this problem, we propose a pose aware confidence (PAC) to filter noisy and inaccurate NOCS pseudo label and additional pose aware self-supervised loss (PAS) to improve the labels. Our PAC and PAS align observed depth to Normalize Object Coordinate Space by leveraging the initial 6D pose and checking outlier of predicted NOCS or minimizing the distances of filtered 3D points. Results show that our PAC and PAS have an advantage in performance compared to the previous UDA methods. Experiments show that our UDA model reaches par with supervised methods and sometimes outperforms strong supervised methods.}

%%%%%%% Origin (do not erase)
%
% Why Category object pose is Necessary instead of Instance level object pose
% 6D object pose estimation is one of the crucial tasks in various robotics and computer vision applications, such as robot manipulation~\cite{zeng2017multi,wong2017segicp,wang2019densefusion,du2021vision} and augmented reality (AR)~\cite{runz2018maskfusion, marchand2015pose, marder2016project}. 
% Previous 6D object pose estimation methods follow the instance-level pose estimation scheme~\cite{tremblay2018deep, xiang2017posecnn, park2019pix2pose, peng2019pvnet, wang2019densefusion, he2020pvn3d, he2021ffb6d} that relies on the given 3D CAD model and the known objects' size information. 
% However, it is not easy to have or obtain accurate 3D scans of every object, and this makes it difficult to apply these algorithms in general settings where the objects have never been seen before, and therefore have no 3D CAD models. Also, it is inefficient to train a separate network for each object and each time a new object is observed.\JS{$\leftarrow$ ??}

% Category-level object pose estimation + NOCS 설명
% To address this problem, category-level object pose estimation has been proposed and gets attention in recently~\cite{wang2019normalized, Tian2020prior, chen2020cass, lin2021dualposenet, wang2021category, chen2021sgpa}. Category-level object pose methods can deal with unseen instances of which only their category is known. Therefore, these methods are more efficient than the instance-level that a single network infers multi-class results at once. Wang~\etal~\cite{wang2019normalized} introduced a new representation called Normalized Object Coordinate Space (NOCS) as a pioneer, to align different object instances within one category in a shared orientation. By predicting a category-wise similar NOCS map, It can estimate the 6D pose of an unseen object without a 3D model.   


% Recent Category-level object pose estimation Problem 
% [Real Labeled Data에 의존 -> 만들기 어렵다.]
% However, Wang~\etal~\cite{wang2019normalized} shows still far performance from satisfactory. Therefore, many improved methods~\cite{Tian2020prior, chen2020cass, lin2021dualposenet, wang2021category, chen2021sgpa} have been proposed recently based on NOCS representation. 
% Tian~\etal~\cite{Tian2020prior} improves NOCS map quality by generating a representative shape-prior and deformation NOCS map for each category. 
% Close to Tian~\etal, CR-Net~\cite{wang2021category} extends the shape-prior method~\cite{Tian2020prior} using cascade relation and recurrent reconstruction method. Similarly, SGPA~\cite{chen2021sgpa} propose the prior adaptation methods to get a stronger prior.  Chen~\etal~\cite{chen2020cass} introduce canonical shape space (CASS) that completes full 3D shape even if it is not visible. \JS{$\leftarrow$ ??}
% Lin~\etal~\cite{lin2021dualposenet} use the NOCS map to boost the performance with refinement. These methods have shown impressive results of category-level pose estimation on RGB-D images. However, these methods require a large number of manual labels including 6D pose and size of objects aligned to RGB and Depth inputs, and NOCS map, which are usually very laborious and costly.


% Real data를 만들기 어려운 것을 해결하기 위한 관련된 방법들 설명 
%   1. Instance level에서의 방법들  
% \TY{Auto-labeling~\cite{zakharov2020autolabeling} tackles single class (car) 3D object detection problem and still does not use full modality (RGB and depth) as network input. 
% Otherwise, we use full modalities as network input for category-level (multi-class) object pose estimation for training and inference.}

%   2. Category-level에서의 방법들
% [기존 방법들의문제 정의] 기존의 방법들은 Complete 3D Shape + Rendering 방법에 의존 -> Complete 3D Shape을 observation만 가지고 reconstruction하는게 어렵다 
% 우리의 방법른 3D shape dependency없이 RGB-D만을 사용해서 이 문제를 해결한다.
% To overcome this problem in the instance-level object pose methods, many works\cite{peng2019pvnet, zakharov2019dpod, kehl2017ssd, park2019pix2pose, wang2020self6d} have tried to render images to get various free 6D pose data using the given 3D CAD models. However, there is significant domain gap (appearance, illumination conditions) between 3D models and real objects and these methods can not deal unseen objects.
% Only a few works~\cite{manhardt2020cps++, zakharov2020autolabeling} have been addressed in category-level object pose. Similar to instance-level, they render image/mask/depth based on the reconstructed 3D shape (mesh~\cite{manhardt2020cps++} or sign distance fields~\cite{zakharov2020autolabeling}) using additional networks \cite{groueix2018papier, park2019deepsdf}. However, estimating unseen 3D shapes from partial observation is a challenge task, and hard to extend multi-class shape estimation with a single network. 
% Therefore, the performance is greatly affected by how accurately and the 3D shape is accurately reconstructed. Moreover, their methods use depth information for a loss function but, they don't fully utilize the RGB-D data and mostly rely on a single RGB for network input. To remedy these problems, the most straightforward solution would be to get rid of the dependency on the complete 3D shape and  utilize RGB-D sensor with domain invariant NOCS representation. 
% Our method can infer object pose and size when an RGB image is not available during inference.



% Ours / UDA-COPE, PAC [Filter 방법, self loss 방법] 강조
% In this paper, we propose a RGB-D based unsupervised domain adaptation for Category-level Object Pose Estimation (UDA-COPE) that address the lack-of-label problem for 6D pose and size, and reduces the domain gap by leveraging the both RGB and depth modality. Inspired by xMUDA~\cite{jaritz2020xmuda}, we use a 3-stream architecture to address the domain gap and self-training strategy with pseudo-labels. Compared to xMUDA, our UDA-COPE uses NOCS representation and focus on how to make high quality pseudo label for category-level pose estimation task. To handle this problem, we propose a pose aware confidence (PAC) to filter noisy and inaccurate NOCS pseudo label and additional pose aware self-supervised loss (PAS) to improve the labels. Our PAC and PAS align observed depth to Normalize Object Coordinate Space by leveraging the initial 6D pose and checking outlier of predicted NOCS or minimizing the distances of filtered 3D points. Results show that our PAC and PAS have an advantage in performance compared to the previous UDA methods. Experiments show that our UDA model reaches par with supervised methods and sometimes outperforms strong supervised methods. 

\end{comment}




% Why Category 6D pose is Necessary
6D object pose estimation is one of the crucial tasks in various robotics and computer vision applications, such as robot manipulation~\cite{zeng2017multi,wong2017segicp,wang2019densefusion,du2021vision} and augmented reality (AR)~\cite{runz2018maskfusion, marchand2015pose, marder2016project}. 
% To recognize and interact with objects in the 3D space, these applications require the types, sizes, locations, and orientations of the objects. For example, for a robot to grasp a mug, it needs to know what kind of a mug it is (type), how big or small the mug is (size), where the mug is exactly lying (location), and in what direction the handle of the mug is pointing (orientation).
% Recent Works [6-DOF] & Current Limitation of Category 6D pose Estimation [Obtaining Labeled data is difficult]


% Although the differential rendering with 3D shapes (mesh, SDF) can generate high-quality synthetic images, the domain gap between and simulated and real environments still exists. From this motivation, Zhang~\etal~\cite{zhang2021keypoint} introduces the Domain Adaptive Keypoints Detection Network (DAKDN) to learn geometry structure and assumes the synthetic and real objects are the same. However, to extend to category-level tasks, the synthetic and real objects are different, it is difficult to expect to learn a consistent geometry structure. For category-level domain gap problem, one potential solution would be using additional depth information to reduce the domain gap. Because It is known that depth information is less affected by domain shift than RGB and most category level methods use depth. Based on this observation, we aim to address the category-level object pose domain shift problem using domain invariant NOCS representation with RGB-D data.




% Ablation study for RGB-D
\begin{table*}
\centering
    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|ccc|cccccccc}
Method       & \begin{tabular}[c]{@{}c@{}}ALL \\ Output Loss\end{tabular} & PAC      & Online Training & 3D IOU (25) & 3D IOU (50) & 3D IOU (75) & 5° 2cm & 5°,5 cm & 10° 2cm & 10°,5 cm & 10°,10 cm \\ \hline
Lower Bound  &                                                            &          &                 & 83.9        & 80.7        & 60.9        & 23     & 27.9    & 57.1    & 67.7     & 69.6      \\ \hline
Pseudo Label &                                                            &          &                 & 84          & 80.3        & 58.6        & 23.8   & 28.2    & 55.9    & 66.5     & 68.4      \\
Pseudo Label & \checkmark                                                   &          &                 & 84          & 81.6        & 60.8        & 24.6   & 29.2    & 54.1    & 64.2     & 66.3      \\
Pseudo Label & \checkmark                                                   & \checkmark &                 & 84.1        & 81.3        & 62          & 28.1   & 32.9    & 55.9    & 65.2     & 67.2      \\
Pseudo Label & \checkmark                                                   & \checkmark & \checkmark        & 84.1        & 82.1        & 61.9        & 30.5   & 35.1    & 56.9    & 66.7     & 69        \\ \hline
Upper Bound  &                                                            &          &                 & 83.9        & 82.9        & 70.4        & 31.8   & 35.8    & 62.2    & 72.4     & 74.5     
\end{tabular}
}
\caption{Ablation study for RGB-D}
    \label{tab:ablation_rgbd}
\end{table*}


To the best of our knowledge, our method is the first work using multi-modal UDA method for the category-level object pose estimation.



% Ablation study fo RGB
\begin{table*}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|cccccccc}
\multirow{2}{*}{Method} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ALL \\ Output Loss\end{tabular}} & \multirow{2}{*}{PAC} & \multirow{2}{*}{Self Loss} & \multicolumn{8}{c}{mAP (↑)}                                                                 \\ \cline{5-12} 
                        &                                                                             &                      &                                  & 3D IOU (25) & 3D IOU (50) & 3D IOU (75) & 5° 2cm & 5°,5 cm & 10° 2cm & 10°,5 cm & 10°,10 cm \\ \hline
Lower Bound             &                                                                             &                      &                                  & 83.3        & 79.9        & 49.7        & 15.4   & 18.3    & 37.6    & 46.7     & 48.9      \\ \hline
Pseudo Label            &                                                                             &                      &                                  & 83.5        & 78.7        & 51          & 11.6   & 13.5    & 36.5    & 42.4     & 44.5      \\
Pseudo Label            & \checkmark                                                                    &                      &                                  & 83.6        & 80.2        & 56.2        & 21.2   & 24.8    & 44      & 50.4     & 52.2      \\
Pseudo Label            & \checkmark                                                                    & \checkmark             &                                  & 83.8        & 81.5        & 59          & 23.3   & 26.1    & 47.7    & 53.1     & 55.1      \\
Pseudo Label            & \checkmark                                                                    & \checkmark             & \checkmark                         & 83.8        & 81.6        & 59.4        & 23.4   & 26.3    & 48.9    & 55.1     & 57.2      \\ \hline
Upper Bound             &                                                                             &                      &                                  & 83.8        & 82.7        & 66.7        & 29.3   & 32.8    & 53.8    & 61.7     & 64.2     
\end{tabular}
}
\caption{Ablation study of RGB branch, Lower Bound(Synthetic Only), Upper Bound (Synthetic + with labeled real data)}
    \label{tab:ablation_study_rgb}
\end{table*}





% Ablation study fo RGB-D
\begin{table*}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc|cccccccc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ALL \\ Output Loss\end{tabular}} & \multirow{2}{*}{PAC} & \multirow{2}{*}{Self Loss} & \multirow{2}{*}{Momentum} & \multicolumn{8}{c}{mAP (↑)}                                                                 \\ \cline{6-13} 
                        &                                                                             &                      &                            &                           & 3D IOU (25) & 3D IOU (50) & 3D IOU (75) & 5° 2cm & 5°,5 cm & 10° 2cm & 10°,5 cm & 10°,10 cm \\ \hline
Lower Bound             &                                                                             &                      &                            &                           & 83.9        & 80.7        & 60.9        & 23     & 27.9    & 57.1    & 67.7     & 69.6      \\
Pseudo Label            &                                                                             &                      &                            &                           & 84          & 80.3        & 58.6        & 23.8   & 28.2    & 55.9    & 66.5     & 68.4      \\
Pseudo Label            & \checkmark                                                                   &                      &                            &                           & 84          & 81.6        & 60.8        & 24.6   & 29.2    & 54.1    & 64.2     & 66.3      \\
Pseudo Label            & \checkmark                                                                   & \checkmark            &                            &                           & 84.1        & 81.3        & 62          & 28.1   & 32.9    & 55.9    & 65.2     & 67.2      \\
Pseudo Label            & \checkmark                                                                   & \checkmark            & \checkmark                  &                           & 84.1        & 82.1        & 61.9        & 30.5   & 35.1    & 56.9    & 66.7     & 69        \\
Pseudo Label            & \checkmark                                                                   & \checkmark            & \checkmark                  & \checkmark                 & 84          & 81.9        & 61.3        & 30.6   & 35.4    & 57.1    & 67       & 69.2      \\
Upper Bound             &                                                                             &                      &                            &                           & 83.9        & 82.9        & 70.4        & 31.8   & 35.8    & 62.2    & 72.4     & 74.5      \\ \hline
\end{tabular}
}
\caption{Ablation study of RGB-D branch, Lower Bound(Synthetic Only), Upper Bound (Synthetic + with labeled real data)}
    \label{tab:ablation_study_rgb}
\end{table*}

==> table/table_metrics/table_pointmixer.tex <==
\begin{table*}[!t]
\setlength{\tabcolsep}{4pt}
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{llccclccccccccccccc}
\Xhline{4\arrayrulewidth}

Method & &
OA & mAcc & mIoU & & 
ceiling & floor & wall & beam & column & window & door & table & chair & sofa & bookcase & board & clutter \\ \Xhline{2\arrayrulewidth}

PointNet & &
- & 49.0 & 41.1 & & 
88.8 & 97.3 & 69.8 & \second{0.1} & 3.9 & 46.3 & 1.8 & 59.0 & 52.6 & 5.9 & 40.3 & 26.4 & 33.2 \\  

PCCN & &
- & 67.0 & 58.3 & & 
92.3 & 96.2 & 75.9 & \first{0.3} & 6.0 & 69.5 & 63.5 & 66.9 & 65.6 & 47.3 & 68.9 & 59.1 & 46.2 \\  

MinkowskiNet & &
- & 71.7 & 65.4 & & 
91.8 & 98.7 & 86.2 & 0.0 & 34.1 & 48.9 & 62.4 & 81.6 & 89.8 & 47.2 & 74.9 & 74.4 & 58.6 \\  

KPConv & &
- & 72.8 & 67.1 & & 
92.8 & 97.3 & 82.4 & 0.0 & 23.9 & 58.0 & 69.0 & 81.5 & 91.0 & 75.4 & 75.3 & 66.7 & 58.9 \\  

% PCTrans~\cite{point-cloud-transformer} & &
% - & 67.6 & 61.3 & & 
% 92.5 & 98.4 & 80.6 & 0.0 & 19.3 & 61.6 & 48.0 & 76.5 & 85.2 & 46.2 & 67.7 & 67.9 & 52.2 \\ 

% CloudTrans~\cite{cloud-transformer} & &
% - & - & 67.9 & & 
% - & - & - & - & - & - & - & - & - & - & - & - & - \\ 

PointTrans & &
\first{90.8} & \second{76.5} & \second{70.4} & & 
\second{94.0} & \first{98.5} & \first{86.3} & 0.0 & \second{38.0} & \first{63.4} & \second{74.3} & \second{89.1} & \first{82.4} & \first{74.3} & \first{80.2} & \second{76.0} & \second{59.3} \\ \Xhline{2\arrayrulewidth}

PointMixer (ours) & &
\first{90.8} & \first{77.4} & \first{71.3} & & 
\first{94.2} & \second{98.2} & \second{86.0} & 0.0 & \first{43.8} & \second{62.1} & \first{78.5} & \first{90.6} & \second{82.2} & \second{73.9} & \second{79.8} & \first{78.5} & \first{59.4} \\ \Xhline{4\arrayrulewidth}

\end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Quantitative results on semantics segmentation in S3DIS dataset.}}
% \vspace{-2mm}
\label{table:semseg}
\end{table*}

==> table/table_metrics/table_sota.tex <==

% Comparison with RGB based supervised state-of-the art methods
\begin{table*}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cccccccc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Syn}      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real Data \\ w/ Labeled\end{tabular}} & \multicolumn{8}{c}{mAP (↑)}                                                                 \\ \cline{4-11} 
                        &                           &                                      & 3D IOU (25) & 3D IOU (50) & 3D IOU (75) & 5° 2$cm$ & 5°,5$cm$ & 10° 2$cm$ & 10°,5$cm$ & 10°,10$cm$ \\ \hline
NOCS (RGB)~\cite{wang2019normalized}              & \checkmark & \checkmark            & 84.80       & 78.00       & 30.10       & 7.20   & 10.00   & 13.80   & 25.20    & 25.8      \\
Shape Prior (RGB)~\cite{Tian2020prior}       & \checkmark & \checkmark            & -           & 75.2        & 46.5        & 15.7   & 18.8    & 33.7    & 47.4     & -         \\ \hline
CPS++ (RGB)~\cite{manhardt2020cps++}             & \checkmark &                                      & 84.6        & 72.8        & -           & -      & 25.2    & -       & -        & 58.6      \\ \hline
Baseline (RGB)              & \checkmark &                                      & 83.6        & 80.2          & 56.2          & 21.2   & 24.8      & 44.0    & 50.4     & 52.2      \\ 
Baseline + xMUDA (RGB)              & \checkmark &                                      & 83.7        & 79.9          & 55.9          & 22   & 24.9      & 45.4    & 50.8     & 52.9      \\ 
Ours (RGB)              & \checkmark &                                      & 83.8        & 82          & 59          & 24.4   & 27      & 49.3    & 54.8     & 56.9      \\
Ours (RGB)              & \checkmark & \checkmark                                      & 83.8        & 82.7          & 66.7          & 29.3   & 32.8      & 53.8    & 61.7     & 64.2      \\ \hline
\end{tabular}
}
\caption{Comparison with RGB based state-of-the art methods that train from synthetic and real datset.}
    \label{tab:real_sota_rgb_comparision}
\end{table*}

% Comparison with RGB-D based supervised state-of-the art methods
\begin{table*}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cccccccc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Syn}      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real Data \\ w/ Labeled\end{tabular}} & \multicolumn{8}{c}{mAP (↑)}                                                                 \\ \cline{4-11} 
                        &                           &                                      & 3D IOU (25) & 3D IOU (50) & 3D IOU (75) & 5°, 2$cm$ & 5°, 5$cm$ & 10°, 2$cm$ & 10°, 5$cm$ & 10°, 10$cm$ \\ \hline
CASS (RGB-D)~\cite{chen2020cass}            & \checkmark            & \checkmark                                                                       & 84.20                & 77.70                & -                    & -               & 23.50            & -                & 58.00             & -                  \\
Shape Prior (RGB-D)~\cite{Tian2020prior}     & \checkmark            & \checkmark                                                                       & 83.40                & 77.40                & 53.50                & 19.50           & 21.60            & 43.50            & 54.00             & 55.8               \\
CR-Net(RGB-D)~\cite{wang2021category}           & \checkmark            & \checkmark                            & -           & 79.30       & 55.90       & 27.80  & 34.30   & 47.20   & 60.80    & -         \\
DualPoseNet (RGB-D)~\cite{lin2021dualposenet}     & \checkmark            & \checkmark                                                                       & -                    & 79.80                & 62.20                & 29.30           & 35.90            & 50.00            & 66.80             & -                  \\
SPGA(RGB-D)~\cite{chen2021sgpa}                                     & \checkmark            & \checkmark                            & -           & 80.10       & 61.90       & 35.90  & 39.60   & 61.30   & 70.70    & -         \\ \hline
Baseline (D)                & \checkmark            &                                                                                 & 83.7                   & 77.1                 & 57.9                 & 18.2            & 24.7             & 46.9             & 64.0              & 65.7               \\
Baseline+xMUDA (D)                & \checkmark            &                                                                                 & 83.8                   & 75                 & 56.1                 & 18.7            & 26.1             & 46.8             & 64.3              & 66.2               \\
Ours (D)                & \checkmark            &                                                                                 & 84                   & 79.6                 & 57.8                 & 21.2            & 29.1             & 48.7             & 65.9              & 68.2               \\
Ours (D)                                     & \checkmark            & \checkmark                            & 83.6           & 79.9       & 64.90       & 23.70  & 29.60   & 55.9   & 69.8    & 71.9         \\ \hline
Baseline (RGB-D)            & \checkmark            &                                                                                 & 84                   & 81.6                 & 60.8                 & 24.6            & 29.2             & 54.1             & 64.2                & 66.3               \\ 
Baseline+xMUDA (RGB-D)            & \checkmark            &                                                                                 & 84                   & 79.5                 & 58.6                 & 24            & 28.5             & 54.7             & 65.1                & 67.2               \\ 
Ours (RGB-D)            & \checkmark            &                                                                                 & 84                   & 82.6                 & 62.5                 & 30.4            & 34.8             & 56.9             & 66                & 68.3               \\
Ours (RGB-D)                                 & \checkmark            & \checkmark                            & 83.9           & 82.9       & 70.4       & 31.8  & 35.8   & 62.2   & 72.4    & 74.5         \\  \hline
\end{tabular}
}
\caption{Comparison with RGB-D based supervised state-of-the art methods}
    \label{tab:real_sota_rgbd_comparison}
\end{table*}

==> table/table_source_only.tex <==
% Source only comparison with state-of-the art
\begin{table*}
\centering
    \resizebox{0.8\linewidth}{!}{
\begin{tabular}{c|cccccccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{8}{c}{mAP (↑)}                                                                 \\ \cline{2-9} 
& 3D IOU (25) & 3D IOU (50) & 3D IOU (75) & 5° 2$cm$ & 5°,5$cm$ & 10° 2$cm$ & 10°,5$cm$ & 10°,10$cm$ \\ \hline
NOCS (RGB)~\cite{wang2019normalized}    & 51.70       & 36.70       & 3.40        & -      & 3.40    & -       & 20.40    & 21.7      \\
CPS++ (RGB)~\cite{manhardt2020cps++}    & 84.5        & 72.6        & -           & -      & 25.8    & -       & -        & 55.4      \\
Shape Prior (RGB-D)~\cite{Tian2020prior}& 81.90       & 71.00       & 43.10       & 11.40  & 12.00   & 33.50   & 37.80    &-           \\ \hline
Ours (RGB)                                                     & 83.3        & 79.9        & 49.7        & 15.4   & 18.3    & 37.6    & 46.7     & 48.9      \\
Ours (D)                                                       & 83.6        & 76.7        & 52.7        & 14.9   & 22.7    & 46.6    & 64.7     & 66.8      \\
Ours (RGB-D)                                                   & 83.9        & 80.7        & 60.9        & 23     & 27.9    & 57.1    & 67.7     & 69.6 \\ \hline
\end{tabular}
}
\caption{Comparison with state-of-the-art methods that train from synthetic dataset.}
    \label{tab:source_only_comparison}
\end{table*}
